On the detection of morphing attacks generated by GANs

Recent works have demonstrated the feasibility of GAN-based morphing attacks that reach similar success rates as more traditional landmark-based methods. This new type of "deep" morphs might require the development of new adequate detectors to protect face recognition systems. We explore simple deep morph detection baselines based on spectral features and LBP histograms features, as well as on CNN models, both in the intra-dataset and cross-dataset case. We observe that simple LBP-based systems are already quite accurate in the intra-dataset setting, but struggle with generalization, a phenomenon that is partially mitigated by fusing together several of those systems at score-level. We conclude that a pretrained ResNet effective for GAN image detection is the most effective overall, reaching close to perfect accuracy. We note however that LBP-based systems maintain a level of interest : additionally to their lower computational requirements and increased interpretability with respect to CNNs, LBP+ResNet fusions sometimes also showcase increased performance versus ResNet-only, hinting that LBP-based systems can focus on meaningful signal that is not necessarily picked up by the CNN detector.

==> Makefile <==
TEXFILE=main.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex
	pdflatex $(@:%.pdf=%.tex); \
	bibtex $(@:%.pdf=%); \
	pdflatex $(@:%.pdf=%.tex); \
	pdflatex --synctex=1 $(@:%.pdf=%.tex)
	mv main.pdf main.synctex.gz build/

all: clean $(PDFFILE)

.PHONY: clean

clean:
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.bbl *.blg
	@rm -vf *.aux *.glo *.dvi *.ps *.pdf *.out *.brf *.fdb_latexmk *.fls *.synctex.gz


==> tables/cross_db_mad_dev.tex <==
\begin{tabular}{llllrl}
       \toprule
              &             &     &          &   AUC &         EER (\%) \\
       Train on & Test on & Extractor & Specs &       &                  \\
       \midrule
       FRLL-SG2 & FRGC-SG2 & Fourier &          &  0.88 &            20.46 \\
              &             & LBP & RIU2 (8,1) $\square$ &  0.93 &            15.16 \\
              &             & CNN & Xception &  0.99 &   \bfseries 5.72 \\
              & FRGC-MIPGAN & Fourier &          &  0.45 &            53.25 \\
              &             & LBP & RIU2 (8,2) $\square$ &  0.96 &            11.39 \\
              &             & CNN & Xception &  0.99 &   \bfseries 5.72 \\
       FRGC-SG2 & FRLL-SG2 & Fourier &          &  0.92 &            16.04 \\
              &             & LBP & RIU2 (8,1) $\square$ &  0.91 &            19.97 \\
              &             & CNN & EfficientNet &  1.00 &   \bfseries 1.20 \\
              & FRGC-MIPGAN & Fourier &          &  0.85 &            23.24 \\
              &             & LBP & (8,2) $\bigcirc$ &  0.99 &             3.91 \\
              &             & CNN & EfficientNet &  1.00 &   \bfseries 0.00 \\
       FRGC-MIPGAN & FRLL-SG2 & Fourier &          &  0.62 &             41.8 \\
              &             & LBP & RIU2 (8,2) $\bigcirc$ &  0.92 &  \bfseries 16.98 \\
              &             & CNN & MobileNet &  0.89 &             19.2 \\
              & FRGC-SG2 & Fourier &          &  0.79 &            28.51 \\
              &             & LBP & (8,2) $\bigcirc$ &  0.97 &             8.76 \\
              &             & CNN & MobileNet &  0.99 &   \bfseries 5.41 \\
       ProGAN & FRLL-SG2 & CNN & ResNet50 &  1.00 &   \bfseries 0.00 \\
              & FRGC-SG2 & CNN & ResNet50 &  1.00 &   \bfseries 0.56 \\
              & FRGC-MIPGAN & CNN & ResNet50 &  1.00 &   \bfseries 0.00 \\
       \bottomrule
       \end{tabular}
       

==> tables/fusion.tex <==
\begin{tabular}{llllllrr}
\toprule
            &          &            &                    Sys. 0 &                     Sys. 1 &  Fused EER (\%) &  Sys. 0 EER (\%) &  Sys. 1 EER (\%) \\
Calibrate on & Test on & Fusion type &                           &                            &                 &                  &                  \\
\midrule
FRLL-SG2 & FRGC-SG2 & All LDA &      RIU2 (8,1) $\square$ &                    Fourier &           10.00 &            15.16 &            20.46 \\
            &          & LBP+ResNet &      RIU2 (8,2) $\square$ &                   ResNet50 &  \bfseries 0.15 &            17.94 &             0.56 \\
            & FRGC-MIPGAN & All LDA &      RIU2 (8,2) $\square$ &  mLBP RIU2 (8,2) $\square$ &           10.98 &            11.39 &            13.09 \\
            &          & LBP+ResNet &          (4,1) $\bigcirc$ &                   ResNet50 &  \bfseries 0.00 &            39.23 &             0.00 \\
FRGC-SG2 & FRLL-SG2 & All LDA &           (4,1) $\square$ &                    Fourier &           12.03 &            19.97 &            16.04 \\
            &          & LBP+ResNet &       U2 (8,1) $\bigcirc$ &                   ResNet50 &  \bfseries 0.00 &            20.99 &             0.00 \\
            & FRGC-MIPGAN & All LDA &          (8,2) $\bigcirc$ &      mLBP  (8,2) $\square$ &            3.65 &             3.91 &             7.90 \\
            &          & LBP+ResNet &  mLBP U2 (8,1) $\bigcirc$ &                   ResNet50 &  \bfseries 0.00 &            26.03 &             0.00 \\
FRGC-MIPGAN & FRLL-SG2 & All LDA &     RIU2 (8,2) $\bigcirc$ &  mLBP RIU2 (8,2) $\square$ &           15.02 &            16.98 &            20.99 \\
            &          & LBP+ResNet &          (8,2) $\bigcirc$ &                   ResNet50 &  \bfseries 0.76 &            19.03 &             0.00 \\
            & FRGC-SG2 & All LDA &          (8,2) $\bigcirc$ &            (4,1) $\square$ &            8.09 &             8.76 &            21.44 \\
            &          & LBP+ResNet &        U2 (8,2) $\square$ &                   ResNet50 &  \bfseries 0.15 &            10.98 &             0.56 \\
\bottomrule
\end{tabular}


==> tables/mad_dev.tex <==
\begin{tabular}{lllll}
\toprule
            &     &                 &             AUC &        EER (\%) \\
Dataset & Extractor & Specs &                 &                 \\
\midrule
FRLL-SG2 & Fourier &                 &            0.92 &           17.31 \\
            & LBP & (8,2) $\bigcirc$ &  \bfseries 0.99 &  \bfseries 5.77 \\
FRGC-SG2 & Fourier &                 &            0.92 &           16.21 \\
            & LBP & (8,2) $\bigcirc$ &  \bfseries 1.00 &  \bfseries 2.86 \\
FRGC-MIPGAN & Fourier &                 &             1.0 &            1.43 \\
            & LBP & (8,1) $\square$ &  \bfseries 1.00 &  \bfseries 0.00 \\
\bottomrule
\end{tabular}

